NeRFiller: Completing Scenes via Generative 3D Inpainting

We propose NeRFiller, an approach that completes missing portions of a 3D capture via generative 3D inpainting using off-the-shelf 2D visual generative models. Often parts of a captured 3D scene or object are missing due to mesh reconstruction failures or a lack of observations (e.g., contact regions, such as the bottom of objects, or hard-to-reach areas). We approach this challenging 3D inpainting problem by leveraging a 2D inpainting diffusion model. We identify a surprising behavior of these models, where they generate more 3D consistent inpaints when images form a 2$\times$2 grid, and show how to generalize this behavior to more than four images. We then present an iterative framework to distill these inpainted regions into a single consistent 3D scene. In contrast to related works, we focus on completing scenes rather than deleting foreground objects, and our approach does not require tight 2D object masks or text. We compare our approach to relevant baselines adapted to our setting on a variety of scenes, where NeRFiller creates the most 3D consistent and plausible scene completions. Our project page is at https://ethanweber.me/nerfiller.

==> extra.tex <==
\section{In-the-wild use cases}

\subsection{Hallucinating Unseen Regions of NeRFs}

Setting: Nerfbusters / Bayes' Rays. We have a training set of images, but we want to render new viewpoints. We define the target novel-view path and then create a dataset to iteratively inpaint.

\subsection{Stepping into 360 RGB-D photos}

Synthetic scenes, Matterport3D 360$^{\circ}$ RGBD Dataset~\cite{rey2022360monodepth} scenes, ...

\textbf{Depth-aware fine-tuning for 360 RGB-D photos.} For stepping into a 360 photo, we use a forward-backward warping technique~\cite{xiang2023ivid} to fine-tune an inpainting model on the photo. This encourages the inpainting model to paint content in-distribution of the scene and to work on depth-aware masks, which might have sharp boundaries due to depth discontinuities.
